A Game-Theoretic Approach to Information-Flow Control via Protocol Composition

In the inference attacks studied in Quantitative Information Flow (QIF), the attacker typically tries to interfere with the system in the attempt to increase its leakage of secret information. The defender, on the other hand, typically tries to decrease leakage by introducing some controlled noise. This noise introduction can be modeled as a type of protocol composition, i.e., a probabilistic choice among different protocols, and its effect on the amount of leakage depends heavily on whether or not this choice is visible to the attacker. In this work, we consider operators for modeling visible and hidden choice in protocol composition, and we study their algebraic properties. We then formalize the interplay between defender and attacker in a game-theoretic framework adapted to the specific issues of QIF, where the payoff is information leakage. We consider various kinds of leakage games, depending on whether players act simultaneously or sequentially, and on whether or not the choices of the defender are visible to the attacker. In the case of sequential games, the choice of the second player is generally a function of the choice of the first player, and his/her probabilistic choice can be either over the possible functions (mixed strategy) or it can be on the result of the function (behavioral strategy). We show that when the attacker moves first in a sequential game with a hidden choice, then behavioral strategies are more advantageous for the defender than mixed strategies. This contrasts with the standard game theory, where the two types of strategies are equivalent. Finally, we establish a hierarchy of these games in terms of their information leakage and provide methods for finding optimal strategies (at the points of equilibrium) for both attacker and defender in the various cases.

==> Makefile <==
all:
	./compile
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.ent
clean:
	rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.ent


==> figure-phases.tex <==
\begin{figure}[t]\label{fig:compositions}
\centering
\begin{picture}(250,150)
%
 \put( 26, 90){$d$}
 \put( 13, 70){\scriptsize $\substack{\mbox{only for}\\[0.6pt]\mbox{visible}\\[0.7pt]\mbox{choice}}$}
 \put( 72, 49){$a$}
 \thicklines \thicklines
 \put(150,140){\framebox(40,15){\Large $\pi$}}
 \put( 58,100){\framebox(50,20){Defender}}
 \put( 58, 59){\framebox(50,25){$\substack{\mbox{Attacker}\\[2.5pt]\mbox{\small ~~~phase 1}}$}}
 \put( 58, 18){\framebox(50,25){$\substack{\mbox{Attacker}\\[2.5pt]\mbox{\small ~~~phase 2}}$}}
 \put(150, 60){\framebox(40,60){\Large $C_{d a}$}}

 \linethickness{0.8pt}
 \put(  40, 110){\line(1, 0){15}}
 \put(  40,  30){\line(0, 1){80}}
 \put(  40,  30){\vector(1, 0){15}}
 \put(  82,  58){\vector(0, -1){15}}
 \linethickness{1.4pt}
 \put( 170, 138){\vector(0, -1){16}}
 \put( 112, 110){\vector(1,  0){32}}
 \put( 112,  70){\vector(1,  0){32}}
 \put( 170,  60){\line(0, -1){30}}
 \put( 170,  30){\vector(-1, 0){58}}
 \put(  82,  17){\vector(0, -1){15}}
 \linethickness{0.6pt}
 \put( 190, 130){\dashbox{1.0}(30,0){}}
 \put( 130,   5){\dashbox{1.0}(90,0){}}
 \put( 220,   5){\dashbox{1.0}(0,125){}}
 \put( 220,  80){\dashbox{1.0}(5,0){}}
%
 \put( 175,127){$x$}
 \put( 175, 40){$y$}
 \put( 125,114){$d$}
 \put( 125, 74){$a$}
 \put(  87,  0){\footnotesize $\substack{\mbox{guess}~ w~~~~~\\[1pt] \mbox{on secret $x$}}$}
 \put( 230, 77){\small Payoff~ $\postvf{\pi}{C_{da}}$}
\end{picture}
\caption{The two phases in a leakage game.}
%\commentMA{I find this figure unnecessary and complicated; actually I'm afraid it makes
%things more confusing for the reader.}
%\replyY{We come back to change this figure if reviewers ask us to put a figure or something like that}
\label{fig:two-phases}
\end{figure}

